Reliable and Efficient Broadcast Routing Using Multipoint Relays Over VANET For Vehicle Platooning

In this paper, we design and implement a reliable broadcast algorithm over a VANET for supporting multi-hop forwarding of vehicle sensor and control packets that will enable vehicles to platoon with each other in order to form a road train behind the lead truck. In particular, we use multipoint relays (MPRs) for packet transmission, which leads to more efficient communication in a VANET. We evaluate the performance based on simulation by running a platooning simulation application program, and show that with MPRs, the communication in the VANET to form a road train is more efficient and reliable.

==> 3_literature.tex <==
\begin{itemize}
% \item Ad hoc relay wireless networks over moving vehicles on highways [\cite{chen2001ad}]
\item VANET Routing Protocols: Review, Implementation and Analysis [\cite{ghori2018vanet}]
\item A comparative study of Various Routing Protocols in VANET [\cite{kumar2011comparative}]
\item VANET based traffic management system development and testing using Aodv routing protocol [\cite{patil2012vanet}]
% \item Intelligent OLSR routing protocol optimization for VANETs [\cite{toutouh2012intelligent}]
% \item A cluster based enhancement to aodv for inter-vehicular communication in vanet [\cite{aswathy2012cluster}]
\item A survey and comparative study of simulators for vehicular ad hoc networks (VANETs)[\cite{martinez2011survey}]
\item VANET routing protocols: Pros and cons [\cite{paul2012vanet}]
% \item Critical Review of Topology Based Routing Protocols in VANETs [\cite{siddiquicritical]}
\item A comparative and analysis study of vanet routing protocols. [\cite{rahem2014comparative}]
\item Simulation based and analysis of routing protocols for vanet using vanetmobisim and NS-2 [\cite{phouthone2015simulation}]
\item  Performance study of various routing protocols in VANET case of study [\cite{ahmed2014performance}]
\item Impact of Node Density and Transmission Range on the Performance of OLSR and DSDV Routing Protocols in VANET City Scenarios [\cite{meraihi2014impact}]
% \item A review of communication, driver characteristics, and controls aspects of cooperative adaptive cruise control (CACC) [\cite{dey2016review}]
\end{itemize}


Rakesh Kumar and Mayank Dav (2012) represent [8], a paper
based on the VANET vehicular ad-hoc networks in wireless
network environment. This is done for the intelligent transportation
system. The applications present in VANET are based upon the data
push communication model. Here the information is disseminated
to set the vehicles. This paper mainly defines the VANET
applications based on the various broadcasting data dissemination
protocols. They are surveyed separately and their fundamental
characteristics are revealed. At the end of this paper comparison of
all the protocols is done and the results are evaluated.
 Amiour med tahar, Bilami azeddine (2007) represent [9], a
paper on VANET vehicular ad-hoc network where vehicles like car,
bus, truck can be assumed as the nodes of the network. The
VANETs routing protocol have a great consequence as the AODV
is one of the most popular routing protocol and is also dedicated to
ad-hoc network. It can use the flooding techniques for locating the
destinations and possibly cause an overhead in the network. This
simulation shows the extended AODV using MPR reduces the load
and performance better than the standard in case of AODVM using
MPR reduces the load and perform better than the standard in case
of traffic with low and high speeds.
 Rakesh Kumar, Mayank Dave represents [10] a paper in (2011)
on vehicular ad-hoc network is subclass of mobile ad-hoc network
which provide a distinguished for intelligent transport system (ITS).
According to the survey it is very necessary to use the ITS with the
help of VANET routing protocol. In paper also discuss the
advantage and disadvantages, applications of different routing
protocols for vehicular ad-hoc networks. This paper also explores
the motivation behind the designed and traces the evolution of this
routing protocol. At last this paper also show the tabular
comparison with various routing protocols for VANET.
 Aswathy M and Tripti represent in the paper [11], in (2012) that
the vehicular ad-hoc networks are special kind of mobile ad-hoc
networks (MANETs). This paper defines the vehicles on road as
nodes of network. With the help of VANET, there are many
applications which are used as an intelligent transportation system.
During the process of route discovery process, AODV broadcasts
route request message (RREQ). It creates many unused routes
between a source and destination node. The main aim of this paper
is to improve the performance of AODV by enhancing the existing 
protocol by creating stable clusters and performing routing by
cluster head and gateway nodes.
 Patil V.P (2012) represents [12] a paper on vehicular ad-hoc
network. This paper suggests more innovative approach to deal with
this traffic congestion problem. This is done by using the
characteristics of Vehicular Ad-hoc Networks (VANET) as a
solution. This system is developed and tested using the AODV
protocol on ad-hoc mobile network to deal with the problem of
vehicle traffic congestion in vehicular network. Traffic congestion
can be measured on the patterns such as packets broadcast,
percentage of packet delivered and percentage of traffic diverted
and overhead to manage the problem of data traffic in the network.
The main simulation shows the domain of vehicle traffic congestion
in which VANET is demonstrated.
 Weiwei Dong (2016) presented [13], that Vehicular ad hoc
network (VANET) is experiencing the frequent link breakage and
low packet delivery rate, which challenges routing protocols. To
address this issue, a Geographic Opportunistic Routing protocol
based on Link state and forwarding quality inside nodes (LF-GOR)
is proposed. LF-GOR improves the transmission reliability and
reduces the delay. The simulation results also demonstrate that in a
highly dynamic network, the packet delivery rate of LF-GOR is
12% higher, the throughput is 1.8kbps higher and the end-to-end
delay is 0.029s lower than that of GyTAR.
 Daxin Tian, (2015) proposed [14], that epidemic routing has
emerged as a promising candidate for giving message dissemination
technique in vehicular ad hoc networks. In this paper, a novel model
is presented to evaluate the capacity of epidemic routing in
vehicular networks with considering the traffic signal control as a
significant factor in urban territory. The review reveals that
epidemic routing can behave differently in different traffic signal
control situations where messages can be forwarded by vehicles
going through the intersections from different directions. The
simulation results prove the accuracy of the model.
 Nikita Mangla (2015) proposed [15], that Vehicular Ad hoc
Networks (VA NETs) allow vehicles to frame a self-organized
network without the requirement for a permanent infrastructure.
The paper also outlined the principle problems which must be
solved for this class of routing protocols and even presented the
solution for the particular problem. The paper will also propose an
algorithm for position based routing at Road Intersection in V
ANETs. The protocols are also compared with respect to the next
proposed routing protocols and accordingly aim at implementing
the following characteristics that are obstacle awareness, street
awareness, no bottleneck and no full path selection.

==> 4_problem.tex <==
In vehicle platooning applications, wireless communication between a lead truck and following vehicles can enable them to form a road train in the highways. Critical sensor and control information such as vehicle position, speed, direction and other related parameters must be exchanged between the lead truck and the following vehicles in order to enable them to automatically maintain the platooning of the several vehicles that are traveling together, where the lead truck will be followed closely by a train of other following vehicles.

Due to the limited range of the communication devices and other propagation characteristics, the wireless devices in different road trains could be spread over a large area forming mobile VANETs. 
The VANET will be used to forward packets from the lead truck to the vehicles at the end of the platoon. Vehicular sensor data packets from the lead truck will be forwarded using the VANET routing protocols through multiple hops of the intermediate wireless devices and eventually to the last few vehicles at the other end of the road train. Sensor data packets from the last vehicles may be forwarded through similar multi-hop paths in the reverse direction to the lead truck.

In the previous chapter, we have taken an overview of five classes of routing protocols in VANETs. In particular, we took a closed looking at several proactive and reactive methods which are widely ackowledged, such as DSR, TORA, AODV, DSDV, and OLSR. The main limitation of these protocols is that they require an explicit route establishment phase before transmission of the data. As we mentioned in Section \ref{sec:bg}, the topology of a VANET changes frequently and unexpectedly due to the high mobility of vehicles, which means the links between vehicles disconnect very often. The frequent route discovery and maintenance not only occupy bandwidth, also lead to severe delay.
As a result, to make sure that the messages could be received reliably and efficiently, \textit{broadcasting} is still the most natural used protocol. In addition, \textit{broadcasting} seems unavoidable in \textit{ad hoc} routing. For instance, both proactive and reactive routing algorithms we mentioned in Chapter \ref{chpt:routing} require to broadcast \texttt{HELLO} messages for neighbor discovery.

Therefore, in this project, we use broadcast protocol for sharing the critical sensor and control information between vehicles in a platoon. 


In this project, sensor and control packets will be transmitted over an emulation of the wireless vehicular ad-hoc network (VANET) that uses an efficient ad-hoc routing protocols. The emulation of the mobile VANET is implemented over a fixed network. The distributed \texttt{tux} machines at the university are used to simulate the experiments. Wireless nodes are executed on different computers, and communicate with each other through the network.

%The following are some design details on how the program is implemented.



\subsection{Vehicle Platooning Application}
A simple road train application program will be implemented to simulate the control for a lead truck and multiple following vehicles, which will enable them to participate in automatic platoon by providing the following functions.
\begin{itemize}
    \item Form a platoon behind a lead truck. 
A vehicle may initiate forming a platoon with a lead truck where the lead truck will determine the road train parameters, e.g. road train speed and direction. Once the platoon is formed, the road train control application will ensure that the following vehicle and the lead truck will travel at the correct speed to
maintain the platoon configuration, i.e. the distance of the gap between the following vehicle and lead truck is within a certain range (e.g., between 10 to 20 meters). 
%We assume that the average speed of each vehicle is 30 meters/sec, with a standard deviation of 10 meters/sec. For more realistic dynamic models, we also assume that the acceleration of the lead truck varies from $-2$ to 2 meter/sec$^2$ randomly. 
The actual speed of each vehicle in a road train may be different. 
    \item Join an existing platoon.
A vehicle that receives vehicle sensor information from other vehicles in the road train may join the road train. Once it joins the road train, it will maintain the road train configuration as above, i.e. it must maintain a spacing from the front and back vehicle of a certain distance (e.g., between 10 to 20 meters).
    \item Leave a platoon. 
A vehicle may leave a road train and need not be bound by the rules for maintaining the road train configuration.
\end{itemize}

% \subsection{Packet Propagation Loss Model}


\subsection{Vehicle Behavior and Packet Categories}
\paragraph*{Vehicle Information Packet Broadcasting}
Every 10 milliseconds, each vehicle will broadcast a packet which containing its own driving information. %to all its one hop neighbors, which are determined through received \texttt{HELLO} messages, as we will illustrate later. 
The datagrams of the vehicle information packets contain the following:
\begin{itemize}
    \item GPS position
    \item Velocity
    \item Acceleration
    \item Brake control
    \item Gas throttle
\end{itemize}

Upon receiving the vehicle information packets from other vehicles, each vehicle would check if the incoming packet is the newest one it has received from the source vehicle (by checking the sequence number). If that is the case, it would update the its own knowledge of the source vehicle if necessary. Also, by checking its MPR selector table, it will know whether to forward/retransmit the received packets with the newest sequence number to all its neighbors, aka every other vehicle in its transmission range (i.e., 100 m), except the one from which it receives the packet (i.e., the previous hop) or the source. The retranmission will be performed if the receiver is selected as an MPR of the previous hop.


% \section{HELLO Messages and MPR Selection}
\subsubsection{Platooning Behavior and Related Packets}
The CACC system needs to be simple, reliable and trustworthy, its primary objective is to maintain a
certain gap in the road train. 
Each following vehicle could join or leave the road train leading by the lead truck by sending \texttt{JOIN} or \texttt{LEAVE} requests. The design of the joining and leaving procedures is one of the key building blocks in our project.

The lead truck sends its driving information to the following vehicles so that the following vehicles in the road train can duplicate its behavior and stay in the road train. The following vehicles send their driving information to the lead truck, so that the lead truck can keep track of their positions, and allow other vehicles to join or leave the road train. The sequence number and the IP address are included in the packet header, and in addition to those \texttt{NORMAL} packets for exchanging the vehicle information, we further define five different types of special packets for controlling the platooning behavior, they are \texttt{JOIN}, \texttt{LEAVE}, \texttt{ACK\_JOIN}, \texttt{NOTIFY}, and \texttt{OK}. 

The following vehicles can send \texttt{JOIN} or \texttt{LEAVE} request to the lead truck, and the lead truck should reply an \texttt{ACK} for that request. 
The \texttt{JOIN} request can only be sent when a following vehicle is not in the road train, i.e., its vehicle state is \textit{FREE}. After it sends a \texttt{JOIN}, the vehicle state becomes \textit{FORM}, which indicates that this vehicle is waiting for the \texttt{ACK\_JOIN} message from the lead vehicle. 
To avoid collision while merging into the middle of the platoon, it is only allowed to join the road train when the lead truck makes sure other vehicles have prepared enough space for it to merge and sends it an \texttt{ACK\_JOIN} message. After it receives \texttt{ACK\_JOIN} and replies with \texttt{ACK\_JOIN}, the vehicle state becomes \textit{FOLLOW}, which indicates that this vehicle has joined the road train, and its driving is controlled by following another vehicle in the road train. It is only allowed to make \texttt{LEAVE} request when it is in the road train, i.e. the vehicle state is \textit{FOLLOW}.
This is like a state machine (See Figure \ref{fig:sm}). Note that in our design, the \texttt{ACK\_JOIN} %and \texttt{ACK\_LEAVE} 
messages sent by the lead truck and by the following vehicle have totally different functionality, the details are described in Section \ref{sec:join}.
While the connection established, the lead and following vehicles communicate their driving information via \texttt{NORMAL} packets.

\begin{figure}
    \centering
    \begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=7.5cm, semithick]
    % \begin{tikzpicture}[->, auto, node distance=5cm, thick]
      \tikzstyle{every state}=[fill=red,draw=none,text=white,minimum size=2.5cm]
    
      \node[initial,state] (A)                    {$FREE$};
      \node[state]         (B) [above right of=A] {$FORM$};
      \node[state]         (C) [below right of=B] {$FOLLOW$};
    
      \path (A) edge [bend left] node { \begin{tabular}{c} 
                            after sending \\ \texttt{JOIN} request \\ to lead truck  \end{tabular} } (B)
            (B) edge [bend left] node { %timeout
                            \begin{tabular}{c} 
                            timeout \\with no \\ \texttt{ACK\_JOIN} \\received  \end{tabular} } (A)
                edge [bend left] node { \begin{tabular}{c} upon receiving \\ 
                            \texttt{ACK\_JOIN} message \\ from lead truck  \end{tabular} } (C)
            (C) edge [bend left] node { %after sending \texttt{LEAVE} request \\ to lead truck} (A) 
                     \begin{tabular}{c} after sending \texttt{LEAVE} request\\ to lead truck \end{tabular} } (A)
                edge [loop below] node {other} (C);
    \end{tikzpicture}
    \caption{Platooning state transitions of vehicles (other than lead truck)}
    \label{fig:sm}
\end{figure}

\subsubsection{Join the Platoon} \label{sec:join}
The specific procedure for the following vehicles to join the road train is as follows:
\begin{itemize}
    \item Initially, only the lead truck stays in the road train. The following vehicles could send request to join the road train at any time if it is not yet in. 
    \item The lead truck then checks the information of the following vehicle that contains in the packet it receives, and determines whether to accept or decline the request of joining the road train, based on if the following vehicle is at the same direction. Once the lead truck decides the following vehicle could have the chance to join the road train, it would then determine which position in the road train the requesting vehicle should join, that is, put the requesting vehicle into the road train right after the nearest vehicle ahead of it, based on the vehicles' current GPS information. If no vehicle in the road train is ahead of it, then it should slow down and follow the lead truck.
    \item If the requesting vehicle were asked to join to the end of the road train, it will then received an \texttt{ACK\_JOIN} message from the lead truck, which tells it which specific vehicle it should follow. If the lead truck determines that the requesting vehicle to join in the middle of the road train, it will inform other vehicles to leave enough space for the joining vehicle first. Only after the vehicle it informed replied an \texttt{ACK} message when enough space has been maintained and thus it is safe to join, the lead truck then sends an \texttt{ACK\_JOIN} to the requesting vehicle.
    \item Once the following vehicle which initiated a \texttt{JOIN} request receives an \texttt{ACK\_JOIN} from the lead truck, it would then accelerate to catch up the platoon, or slows down for waiting the platoon, until reaches a desired location so that it keeps an appropriate distance from the vehicle in front of it in the road train, it would then moves to the right lane of the road, set the speed and acceleration in order to follow the vehicle in front of it, upon the information received from that vehicle most recently. Remark that to simplify the model, we assume the acceleration/de-acceleration to the desired speed for catching up or slow down is instantaneous, so is the braking and moving to the right lane and joining the platoon.
    \item After joining the road train, the requesting vehicle sends an \texttt{ACK\_JOIN} to the lead truck. The lead truck then update its own knowledge about the road train topology, and could be able to process the next \texttt{JOIN} or \texttt{LEAVE} request.
\end{itemize}

The above procedures are depicted in Figure \ref{fig:j1} and Figure \ref{fig:j2}, which illustrate different situations whether the following vehicle is about to join to the end or middle of the road train, respectively.

\begin{figure}[htb!]
    \centering
    \includegraphics[width=\textwidth]{figs/join1.PNG}
    \caption{Procedure for a following vehicle joining the road train to the end}
    \label{fig:j1}
\end{figure}
% \clearpage

\begin{figure}[htb!]
    \centering
    \includegraphics[width=\textwidth]{figs/join2.PNG}
    \caption{Procedure for a following vehicle joining the middle of the road train}
    \label{fig:j2}
\end{figure}
% \clearpage

\subsubsection{Leave the Platoon}
For a following vehicle to leave the road train, the procedure is much simpler. The following vehicle $k$ sends a \texttt{LEAVE} message to the lead truck, without the need of receiving any response, it then moves to the left lane, and is no longer be controlled by the road train. To increase the reliability of the communication, we let the leaving vehicle sends \texttt{LEAVE} message for three times. Once the lead truck receives the \texttt{LEAVE} packet, it needs to inform the vehicle ($k+1$) in the road train which was following the left vehicle $k$ to follow the one previously was ahead the left one, (i.e., $k+1$ should follow $k-1$ instead of $k$ after $k$ leaves), by sending a \texttt{NOTIFY} message to vehicle $k+1$. This information can be calculated from the road train topology table cached in the lead truck, and upon receiving the \texttt{LEAVE} message, the lead truck need to update its knowledge about the road train topology.
The informed vehicle, as well as all other vehicles behind it, then speed up a little and fill up the space. 
Note that the only information that the lead truck notifies the informed vehicle is which vehicle in the road train it should follow, and the informed vehicle changes its speed based on its own knowledge about other vehicles' driving information from corresponding \texttt{NORMAL} packets it received. 
%It then sends back an \texttt{ACK} to the lead truck, so that the lead truck could updates its own knowledge about the road train topology, and is able to process the next \texttt{JOIN} or \texttt{LEAVE} request. Note that before receiving the \texttt{ACK} message from the informed vehicle, all other received \texttt{JOIN} or \texttt{LEAVE} requests will not be processed by the lead truck, but will be cached in a queue. In other words, they will be processed in FIFO sense. 

\subsection{Packet Forwarding Protocols}
In order for a vehicle to learn about the position, speed and acceleration of road train and other cars, each vehicle and the lead truck must transmit its sensor data containing its GPS position, speed and acceleration at a constant period of 10 to 100 milliseconds. These sensor data are then forwarded multi-hop. In this section, we will design two schemes of broadcasting, one uses MPRs while the other one does not. Both algorithms aims at reliably sending information packets to other vehicles. The network broadcast protocols will be built on top of the simple UDP (User Datagram Protocol) socket interface that emulates the wireless link layer. The structure is shown as in Figure \ref{fig:struct}. Note that the wireless link layer is not part of this project, but represents protocols that could conceptually be added or substituted.

\begin{figure}[hb]
    \centering
    \begin{tikzpicture}
        \filldraw[fill=gray!40!white, draw=black] (0,0) rectangle (6, 2) node[pos=.5] { 
            \begin{tabular}{c} Wireless Link Layer \\ (UDP Datagrams)
            \end{tabular}
        };
        % \draw (0,2) rectangle (6, 6) node[pos=.5]{Network Broadcast Protocol};
        \filldraw[fill=yellow!5!white, draw=black]  (0,2) rectangle (6, 6);
        % \draw (0,2) rectangle (6, 6);
        \node at (3, 5) {Network Broadcast Protocol};
        \filldraw[fill=red!5!white, draw=black] (1.5,3.5) ellipse (1 and .5) node{RBA};
        \filldraw[fill=red!5!white, draw=black] (4.5,3.5) ellipse (1 and .5) node{MPR};
        \node at (3,3.5) {or};
        \filldraw[fill=green!5!white, draw=black]  (0,6) rectangle (6, 8) node[pos=.5]{Road Train Application};
    \end{tikzpicture}
    \caption{Overview of the VANET Protocols Components}
    \label{fig:struct}
\end{figure}


\subsection{Reliable Broadcast Algorithm}
We first design a \textit{reliable broadcast algorithm} (RBA) on top of the link layer. 
Initially, each vehicle will generate a vehicle sensor packet depending on its dynamics and forwards it to all its neighbor nodes through its RBA layer. Eventually the packet will be forwarded through multiple hops and reach all other vehicle destination addresses. The RBA layer of the intermediate nodes performs the task of forwarding packets reliably from one node to another. The packet header must contain at least the following fields:
\begin{enumerate}
    \item Sequence number
    \item Source address
    \item Previous hop (address)
\end{enumerate}

Each vehicle node will run the program for the RBA as follows.  
In the RBA layer, each vehicle maintains a \textit{cache table} of the broadcast packets that it has received from every other source node in the network, with the largest sequence number of the packets that it has received from the source up to that time point, i.e. the \textit{cache table} contains information on broadcast packets that the node has forwarded previously. Now for a node with address $addr_i$, consider the case it receives a packet from another node with address $addr_{prev}$, which can be examined from the \textit{``Previous Hop''} field specified in the packet header,  it will first check the source address $addr_s$ of the received packet. If the packet source is itself ($addr_s=addr_i$), the packet will be discarded; otherwise it then compares the sequence number $sn_p$ of the packet with the largest sequence number $sn_s$ it cached for source $addr_s$ in its \textit{cache table}. 
%If the sequence number in the \textit{cache table} is larger than or equal to that of the received packet, i.e. $sn_s \ge sn_p$, which means this node has received this packet or newer ones from the source before, so this packet will also be discarded; 
If there is no $sn_s$ record in the \textit{cache table}, or the sequence number in the \textit{cache table} is smaller than that of the received packet, i.e. $sn_s<sn_p$, which means this packet is the newest from source $addr_s$ for node $addr_i$, and needs to be forwarded. The node with $addr_i$ will then update its cache table, in which the sequence number from source $addr_s$ is replaced by $sn_p$, and the \textit{broadcast number} $bn$ for that packet is set to 1. In addition, it changes the \textit{``PrevHop''} field of the packet to its own address $addr_i$, and forwards a copy of the packet to each of its neighbors except the one from which it received this packet, i.e., $addr_{prev}$. Eventually the packet is sent to all the reachable wireless nodes. 

To ensure the reliability of the broadcast protocol, we also design a \textit{re-broadcasting} mechanism for increasing the redundancy, in case the previous broadcast packet was lost. With \textit{re-broadcasting}, 
if the sequence number in the \textit{cache table} is the same as that of the received packet, i.e. $sn_s \ge sn_p$, the \textit{cache table} will also be updated, by adding one to the \textit{broadcast number} of that packet. And that packet may be forwarded depending on the probability determined by the \textit{broadcast number}, which in fact records the number of times the same packet has been re-broadcasted. If the packet has been broadcast once, there is a 50\% probability of re-broadcasting it to its neighbors; if it has been broadcasted twice, then the probability is 25\%, and so on.



\subsection{Broadcasting with MPRs}
Alternatively, a broadcast protocol using MPRs on top of the link layer will be designed and implemented. 
In this protocol, each vehicle continuing broadcasts \texttt{HELLO} messages which contain its own one hop neighbors as well as their link status every 20 milliseconds, and we assume that any other
vehicles could receive the packets only when their distance is within 100 m. The link status
of each one hop neighbor could be either uni-directional, bi-directional, or MPR.

Upon receiving \texttt{HELLO} messages from others, each vehicle is able to learn the knowledge of its neighbors up to two hops. After sensing the neighbors, the \texttt{HELLO} message receiver then could have enough information to select its MPRs from its bi-directional linked one hop neighbors, by knowing all its two hop neighbors (as well as their access through nodes). The \texttt{HELLO} message receiver then could update all the neighborhood information in its \textit{neighbor table}, which contains its one hop neighbors, the status of the link with these neighbors, and a list of two hop neighbors that these one hop neighbors give access to, as well as a sequence number which specifies the most recent MPR set that the local node keeping this neighbor table has selected. Every time a node selects or updates its MPR set, this sequence number is incremented to a higher value. Moreover, on reception of \texttt{HELLO} messages, each vehicle is able to know is this one hop neighbor has selected it as an MPR or not. Based on that, it can construct a MPR selector table, so that it will know whether to retransmit the received packets (other than \texttt{HELLO} messages). 

Every broadcast message coming from these MPR Selectors of a node is assumed to be retransmitted by that node. This set can change over time, which is indicated by the selector nodes in their \texttt{HELLO} messages.

\subsubsection{Neighbor Sensing and MPR Selection}
After receiving \texttt{HELLO} messages, the receiver vehicle (let us denote it as $R$) might need to update its neighborhood information. First of all, we need to check whether the sender (we denoted it as $S$) was $R$'s two-hop neighbors previously, it needs to be removed if it is the case. 
In any case, $S$ should then be added into $R$'s one-hop neighbors if it was not there, and the link will be set as uni-directional if $R$ has not been declared as $S$'s one hop neighbor in this \texttt{HELLO} message. On the other hand, in the \texttt{HELLO} message, if $R$ is already $S$'s one hop neighbor, then the link for $S$ will be set as bi-directional. 

Next, we need to update $R$'s two-hop neighbors information. Note that each of $R$'s two-hop neighbor ($M$) will maintain a set to record through which $R$'s one-hop neighbor, $M$ could get access through and reach $R$. Also note that the received \texttt{HELLO} contains the link status of all $S$'s one-hop neighbors, upon which $R$'s \textit{MPR selector table} could be updated. Moreover, if $S$ was already a bi-directional one-hop neighbor for $R$, then there might exist some $M$  which use $S$ as an access through point to get to $R$. But if now the bi-link between $S$ and $M$ was unlinked (as specified in the received \texttt{HELLO}), in that case, we need to remove $S$ from $N$'s access through set, and we need to traverse the two-hop neighbors and do this for all possible $M$'s. If any such $M$ has empty access through set after removing (i.e., $S$ was the sole access through point for $M$ to reach $R$), it will also be cleaned from $R$'s two-hop neighbors.

We also need to traverse for each of $S$'s one hop neighbor $N$, which could be a candidate for $R$'s two hop neighbor. 
If $N$ is already a two hop neighbor of $R$, we need to update $N$'s access through set by adding source if necessary. Otherwise, $N$'s access through set will be newly constructed and contains only $S$, with that information, $N$ is then added as a new two-hop neighbor for $R$.

If there is any change, $R$'s MPRs need to be selected again. We use heuristics for MPR selection. First we sort the two hop neighbors by the number of one-hop neighbors (called access-through set $\mathcal{A}$, in which the element is denoted as $A$) they connected with (note that the connection must be bidirectional). Then we allow the one with the fewest links with the access-throughs ($A$'s) chooses its MPR first, by randomly choose an element in $\mathcal{A}$; Then the one with second-fewest $A$'s; and so on, until all two-hop neighbors are traversed.

Lastly, we update the one-hop neighbors by labeling their link status. If a one-hop neighbor has been selected as an MPR, we label its link status as MPR. However, if a one-hop neighbor was an MPR previously, but has not been selected this time, we need to degrade its link status as bi-directional. 

\begin{table}[htb]
    \centering
    \begin{tabular}{|c|c|}
    \hline \hline
\multicolumn{2}{|c|}{Node 4's One-Hop Neighbors}  \\ \hline
Node ID & Status \\
\hline
   3   &   MPR  \\
    5   &    MPR   \\
    6   &    BI   \\
    7   &   BI  \\
    8   &   BI  \\
    9  &    BI  \\
\hline \hline
\multicolumn{2}{|c|}{Node 4's TWO-Hop Neighbors}  \\ 
\hline 
 Node ID &   Access Through (MPR) \\
\hline 
    1    &     3  \\
    2     &    3  \\
    10    &    5  \\ \hline \hline
    \end{tabular}
    \caption{Exemplary Neighbor Table}
    \label{tab:nbTab}
\end{table}

A typical neighbor table would be like in Table \ref{tab:nbTab}, which is obtain from our experiment for 10 vehicles in the VANET.

\subsubsection{OLSR Protocol for Special Packets}
Those 7 types of special packets for joining and leaving the road train are the only packets use the optimized linked state routing (OLSR) protocol, since they are the only packets that specify the destination. The OLSR protocol is based on MPR selection, which we have already illustrated. The MPRs will send topology control (\texttt{TC}) messages to all its one hop neighbors every 30 milliseconds, in which only its own MPR selector table is declared. The sequence numbers of \texttt{TC} just use the sequence number of the neighbor table in that vehicle, so even new \texttt{TC} messages are generated, if no neighborhood information is changed, the sequence number would not increase. 

The \texttt{TC} messages are used for every vehicles in the network to update their \textit{topology tables}. Each vehicle maintains its own \textit{topology table}, which has an entry for each of the other vehicles it knows in the network. Each entry contains some information about the initiator of the \texttt{TC} messages, which includes the address, MPR selectors, the largest sequence number of received \texttt{TC} messages from the initiator, and a holding time. Upon receiving an \texttt{TC} message, the corresponding entry is updated only when the \texttt{TC} message is larger than the one saved in the \textit{topology table}. And if the two sequence numbers are equal, the holding time of that entry will be refreshed.

The \textit{topology table} is used for updating the \textit{routing table}, from which the vehicle could calculate which the next hop is for sending or forwarding those 7 types of special packets. The calculation of next hop requires keeping track of a reversed path from the destination through its MPRs, to the MPRs' MPRs if necessary, until one of the vehicle's one hop neighbor. \textit{Bread First Search} is used for the calculation.

By doing above procedures, $R$'s neighborhood information as well as MPR selector table have been updated. If there is any change, the neighbor table sequence number will be increased, and the routing table will also be updated. The neighborhood information will be used for sending and forwarding packets, and also would be written into new \texttt{HELLO} messages. The MPR selector table would be transmitted to other vehicles if it is an MPR. 

\subsection{Network Configuration}


% \section{Configuration File}
The status of each packet sending and receiving would be recorded into a configuration file. %Upon which we could calculate the performance of the network, including the statistics of throughput, packet loss rate, latency, etc.
A configuration file helps us to look at the link state between the vehicles, also the status of each sent or received packet. The vehicles write information into the configuration file, but do not track and utilize information from it. The configuration file looks like as in Table \ref{tab:my_label}.

\begin{table}[h]
    \centering
    \begin{tabular}{c c c r r l}
    \hline  \hline
        Node 1 & tux055, & 10010 & 50 & 120 & links 2 \\
        Node 2 & tux055, & 10011 & 80 & 120 & links 1 3 4\\
        Node 3 & tux060, & 10010 & 180 & 170 & links 2 4\\
        Node 4 & tux060, & 10011 & 150 & 60 & links 2 3\\
         \multicolumn{6}{c}{$\cdots \cdots$} \\
    \hline
    \end{tabular}
    \caption{Exemplary Configuration File}
    \label{tab:my_label}
\end{table}

\subsection{Simulation set-up}
To simulate different number of vehicles in a road train, the program needs to run on different tux machines. As there is no physical access to tux machines, remote login is needed. Multiple remote login windows may be necessary. The lead truck should always be instantiated first, and when the program starts to run, the lead truck will first erase the configuration file if that exists, and then write its own information into the file. The configuration file helps to track the existing nodes in the simulation environment, as well as their link states. Only after the lead vehicle were added into the environment, other vehicles, aka following vehicles, could enter the simulation. Each of the vehicle would have a unique node ID, starting from 1 for the lead truck, and incrementally generated for every vehicles when they were added. Each vehicle continues broadcasting \texttt{HELLO} messages which can be received by all other vehicles within a certain transmission range (i.e., 100 meters) with a loss rate. Upon that, each vehicle could maintain a neighbor table and select MPRs. Each vehicle continues sending packets containing information about its status to all its one hop neighbors, among which only MPRs will retransmit the received vehicle information packets. In this way, all other vehicles are able to sense the information by receiving the packets if they are within the transmission range of any vehicle. Following vehicles can make \texttt{JOIN} and \texttt{LEAVE} request depending on if they are in the road train, through \textit{optimized linked state routing} (OLSR) protocol. Note that all packet are sent and received among vehicles by using use UDP protocol. 


